Delta-Decision Procedures for Exists-Forall Problems over the Reals

Solving nonlinear SMT problems over real numbers has wide applications in robotics and AI. While significant progress is made in solving quantifier-free SMT formulas in the domain, quantified formulas have been much less investigated. We propose the first delta-complete algorithm for solving satisfiability of nonlinear SMT over real numbers with universal quantification and a wide range of nonlinear functions. Our methods combine ideas from counterexample-guided synthesis, interval constraint propagation, and local optimization. In particular, we show how special care is required in handling the interleaving of numerical and symbolic reasoning to ensure delta-completeness. In experiments, we show that the proposed algorithms can handle many new problems beyond the reach of existing SMT solvers.

==> discussion.tex <==
Compare decision problem with QE?

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> preamble.tex <==
%\usepackage{multirow}
% \usepackage{amsmath,hyperref}
% \hypersetup{
%     colorlinks,%
%     citecolor=blue,%
%     filecolor=blue,%
%     linkcolor=blue,%
%     urlcolor=blue
% }
\usepackage{amssymb,verbatim}
\usepackage{fix2col,listings,fancyvrb}
\usepackage{multicol}
\usepackage{graphicx,epsfig}
\usepackage{caption}
\usepackage{stmaryrd}
\usepackage{setspace}
\usepackage{ulem}
\usepackage{newlfont}
\usepackage{epsfig,graphics}
\usepackage{fancybox}
\usepackage{listings}
\usepackage{caption}
\usepackage{graphicx,epsfig}
\usepackage{caption}
\usepackage{makeidx}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{listings}
\lstset{
  basicstyle=\ttfamily,
  breaklines=true,
  columns=fullflexible,
  escapeinside = ||,
  breakindent=0pt}
\makeindex

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{hyperref}
\hypersetup{
    colorlinks,%
    citecolor=blue,%
    filecolor=blue,%
    linkcolor=blue,%
    urlcolor=blue
}
\usepackage{multicol}
\usepackage{lipsum}

\newtheorem{theorem}{Theorem}
\newtheorem{proofoutline}[theorem]{Proof Outline}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{question}[theorem]{Question}


%\usepackage[ruled,lined,boxed,commentsnumbered,linesnumbered]{algorithm2e}

\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{2}

\newcommand\bookepigraph[4]{
\vspace{1em}\hfill{}\begin{minipage}{#1}{\begin{spacing}{0.9}
\small\noindent\textit{#2}\end{spacing}
\vspace{1em}
\hfill{}{#3}\\

\vspace{-1em}\begin{flushright}{#4}\end{flushright}}\vspace{2em}
\end{minipage}}

\newcommand{\dom}{\mbox{dom}}

\newcommand\epigraph[3]{
\vspace{1em}\hfill{}\begin{minipage}{#1}{\begin{spacing}{0.9}
\small\noindent\textit{#2}\end{spacing}
\vspace{1em}
\hfill{}{#3}}\vspace{2em}
\end{minipage}}

\newcommand\anonymousepigraph[2]{
\vspace{1em}\hfill{}\begin{minipage}{#1}{\begin{spacing}{0.9}
\small\noindent\textit{#2}\end{spacing}}
\vspace{1em}
\end{minipage}}

\newcommand{\len}{\mathit{len}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\cf}{\mathsf{CF}}
\newcommand{\be}{\mathsf{BE}}
\newcommand{\fe}{\mathbb{F}^{[\underline{e}, \overline{e}]}_{\beta,p}}
\newcommand{\rad}{\mathrm{rad}}


\newcommand{\flow}{\mathsf{flow}}
\newcommand{\jump}{\mathsf{jump}}
\newcommand{\inv}{\mathsf{inv}}
\newcommand{\init}{\mathsf{init}}
\newcommand{\guard}{\mathsf{guard}}
\newcommand{\reset}{\mathsf{reset}}
\newcommand{\reach}{\mathsf{Reach}}
\newcommand{\unsafe}{\mathsf{unsafe}}

\newcommand{\safe}{\mathsf{safe}}
\newcommand{\p}{\mathsf{P}}
\newcommand{\np}{\mathsf{NP}}
%\newcommand{\dom}{\mathrm{dom}}


\newcommand\tupleof[1]{\left\langle #1 \right\rangle}
\newcommand\vI{\vec{I}}
\newcommand\va{\vec{a}}
\newcommand\vb{\vec{b}}
\newcommand\vc{\vec{c}}
\newcommand\vd{\vec{d}}
\newcommand\ve{\vec{e}}
\newcommand\vl{\vec{l}}
\newcommand\vu{\vec{u}}
\newcommand\vx{\vec{x}}
\newcommand\vy{\vec{y}}
\newcommand\trp[1]{#1^{{}^{\mbox{\sc{t}}}}}
\newcommand{\lrf}{\mathcal{L}_{\mathbb{R}_{\mathcal{F}}}}
%\usepackage{wrapfigure}

%\doublespacing


==> table1.tex <==
\begin{table}
  \centering
  \begin{tabular}{|l|l|l|l||l|l|l|l|l|l||l||l|}
    \hline
    \multicolumn{4}{|c||}{Problem}    & \multicolumn{6}{c||}{Our Implementation (based on dReal3)}                                & Z3   & CVC4\\
    \hline
    Name        & Constraints &\#EV & \#UV & \#BR & \#PR & \#CE & $\delta$ & Time & $\mathrm{Time}_L$ & Time & Time\\
    \hline \hline
    testtube    & $\sin,\cos,\exp$ & 2 & 2    & 39   &  742 & 15   & 1e-5     & 0.028& 0.030             & N/A  & N/A\\  % 148
    rosenbrock  & poly-4 & 3 & 3    & 88   & 1890 & 11   & 1e-3     & 0.045& 0.017             & N/A  & N/A\\
    beales      & poly-6 & 2 & 2    & 73   &  1685& 63   & 1e-3     & 0.057& 0.029             & N/A  & N/A\\
    bohachevsky & $\cos$ & 2 & 2    & 22   & 404  & 9    & 1e-4     & 0.022& 0.006             & N/A  & N/A\\
    eggholder   & $\sin, \sqrt{\cdot}, |\cdot|$   & 2 & 2    & 8063 &272292& 2    & 1e-4     & 1.833& 1.690             & N/A  & N/A\\
    zettl       & poly-4   & 2 & 2    & 1453 &408365& 4011 & 1e-5     & 1.897& 2.645             & N/A  & N/A\\  % 174
    multi       & $\sin,\cos$   & 3 & 3    & 55   & 1082 & 32   & 1e-3     & 0.049& 0.048             & N/A  & N/A\\  % multi-14
    gams        & poly-2 & 4 & 4    & 336  & 20160& 24   & 1e-3     & 0.402& 0.249             & N/A  & N/A\\
    wall        & poly   & 6 & 6    & 1511 & 97297& 19   & 1e-2     & 29.070& 27.349           & T/O  & N/A\\
    abel        & poly-2   &30 &30    & --   & --   & --   & --       & T/O   & T/O              & N/A  & N/A\\
    \hline
  \end{tabular}
  \caption{Experimental Results: \#EV: exist-vars, \#UV: forall-vars,
    \#BR: branchings, \#PR: prunings, \#CE: counterexamples,
    $\mathrm{Time}$: running time, $\mathrm{Time}_L$: running time with local-optimization, T/O: timeout(10min)}
  \label{table:experiments}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> table2.tex <==
\begin{center}
\begin{tabular}{l|rrrrrr}
 & \#V & \#C & \#CE & \#Br & Prec & Time\\
\hline
\hline
D1 & 6 & 10 & 40 & 10 & 0.001 & 0.33\\
D2 & 6 & 10 & 97 & 32 & 0.001 & 1.42\\
D3 & 2 & 4 & 7184 & 2052 & 0.001 & 147.68\\
D4 & 3 & 6 & 80 & 22 & 0.001 & 0.24\\
D5 & 6 & 4 & 76 & 39 & 0.05 & 12.44\\
D6 & 6 & 11 & 53 & 19 & 0.5 & 12.77\\
D7 & 6 & 10 & 155 & 115 & 0.001 & 2.67\\
D8 & 6 & 10 & 185 & 40 & 0.001 & 1.68\\
D9 & 6 & 10 & 99 & 40 & 0.001 & 1.24\\
D10 & 6 & 4 & 60 & 19 & 0.001 & 0.31\\
D11 & 6 & 4 & 305 & 39 & 0.025 & 102.68\\
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{l|rrrllrl}
 & \#V & \#C & \#O & \#CE & \#Br & Prec & Time\\
\hline
\hline
M8 & 6 & 6 & 2 & --- & --- & 0.05 & T/O\\
M9 & 4 & 8 & 4 & 992 & 105 & 0.001 & 42.14\\
M10 & 4 & 4 & 5 & --- & --- & 0.001 & T/O\\
\end{tabular}
\end{center}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

